Integrating Accessibility in a Mobile App Development Course

The growing interest in accessible software reflects in computing educators' and education researchers' efforts to include accessibility in core computing education. We integrated accessibility in a junior/senior-level Android app development course at a large private university in India. The course introduced three accessibility-related topics using various interventions: Accessibility Awareness (a guest lecture by a legal expert), Technical Knowledge (lectures on Android accessibility guidelines and testing practices and graded components for implementing accessibility in programming assignments), and Empathy (an activity that required students to blindfold themselves and interact with their phones using a screen-reader). We evaluated their impact on student learning using three instruments: (A) A pre/post-course questionnaire, (B) Reflective questions on each of the four programming assignments, and (C) Midterm and Final exam questions. Our findings demonstrate that: (A) significantly more ($p<.05$) students considered disabilities when designing an app after taking this course, (B) many students developed empathy towards the challenges persons with disabilities face while using inaccessible apps, and (C) all students could correctly identify at least one accessibility issue in the user interface of a real-world app given its screenshot, and 90% of them could provide a correct solution to fix it.

==> findings.tex <==
% !TeX root = main.tex

\section{Findings}
\label{sec:findings}

% The assessments exhibit that the core learning objectives that were set out for the course were successfully met. In this section, we discuss the various findings related to integrating accessibility and its outcome in the course. As mentioned in the previous section, we used three instruments to assess the students across the parameters of Accessibility Awareness, Technical Skills, and Empathy. We report the findings from each instrument below, followed by a discussion on our interpretation of the results obtained.

Data collected from all three instruments ---the open-ended questionnaire, the reflective questions on the assignments, and the exam questions--- is qualitative text data. 
We followed the methods of Salda\~na~\cite[pp.~115--121]{saldanaCodingManualQualitative2021} to perform Mangnitude Coding on each data set. 
In each case, two researchers independently identified codes from 10\% of the sample and agreed on the definitions of the codes before classifying the rest of data using those codes.

\subsection{Inclusive Thinking Questionnaire}

% Each student response was coded for the presence of one or more of these four factors we considered for inclusive thinking:
% \begin{itemize}
%     \item \texttt{DIS}: considering disabilities when designing the app, e.g., user-testing the prototype with persons with disabilities;
%     \item \texttt{TECH}: considering alternatives due to limited access to technology for certain sections of the population, e.g., using text messaging to validate vaccination in addition to data messages to handle the lack of availability of high-speed internet in some areas;
%     \item \texttt{SOCIAL}: considering various social factors when designing the app, e.g., user-testing the prototype with various age groups and socio-economic backgrounds;
%     \item \texttt{LANG}: considering the language barrier, particularly the lack of English-proficiency, e.g., providing the app in other Indian languages.
% \end{itemize}


% For each factor, we have a dichotomous dependent variable (e.g., \texttt{DIS} with levels `present' and `not present') and we have taken repeated measurement. So we use McNemar's Test~\cite{pemburysmithEffectiveUseMcNemar2020} to determine if there was a significant difference between the pre- and post-questionnaire for each factor.



% namely disabilities, access to technology, age and literacy, and language barrier. Since our categorical variables represent "pre-course" and "post-course" observations, the $\chi^2$ test of independence is not appropriate as the assumption of the independence of observations is violated. Hence, a McNemar's Test has been used. The responses ($n=40$) were distributed into codes based on the forms of inclusivity considerations they talked about. In the pre-course survey, it was found that only 2.5\% of students mentioned disabilities, while 42.5\% mentioned access to technology, 35\% age and literacy, and 10\% considered language barrier while responding to this questionnaire. 

% At the end of the course, it was found that 42.5\% of students mentioned disabilities, 52.5\% mentioned access to technology, 32.5\% age and literacy, and 12.5\% language barrier.
% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=10cm]{prepostGraph.png}
%     \caption{Comparison of Pre-course and Post-course Questionnaire Results }
%     \label{fig:prepost}
% \end{figure}
% A Statistically significant difference was found between pre- and post-course results on the disabilities category with p=0.000031 (p<0.05 and two-tailed) and no significant differences was found between pre- and post-course results on the other three categories: access to technology (p=0.42395, two tailed) age and literacy(p=1, two tailed) and language barriers (p=1, two tailed). 

\subsection{Findings from the Reflective Questions on the Programming Assignments}


% The accessibility-related tasks were worth 5 points in A1, and worth 10 points each in A2 and A3. The table also shows average score on the accessibility-related tasks, scaled to 10, for each assignment.

% There were four assignments for the course. For these assignments, we analyzed the accessibility portion of the students' written responses, where they had self reported their experiences trying out assistive technology, and their approach towards UI testing keeping accessibility in mind. As mentioned in the methodology section, these were analyzed by coding the responses into various categories by two researchers as indicated in the methodology section.
% In the first assignment, out of the 56 responses, 96\% of them reported having explored their app using \tb{} and 94\% of students reported to have used the accessibility scanner on their application. Some interesting findings are that around 19\% of them also radiated a sense of empathy towards PwD and the importance of accessibility. In the first assignment, students also felt that using assistive technologies like talkback and accessibility scanner requires a learning curve and 53\% of the responses conveyed that they found it difficult and challenging to use talkback.
% \newline
% In the second assignment, out of the 56 respondents, 17\% of the responses indicated empathy and 21\% of them indicated that students are cautious of accessibility issues and choose appropriate colors and labels during design and development of the application.
% \\ 
% In the third assignment and fourth assignment, though accessibility was not a part of the rubric, 44\% and 46\% of the responses indicated that students care about accessibility and ran UI/accessibility tests. 

% \subsection{Findings from the Exam Questions}

